Multi-User Chat Assistant (MUCA): a Framework Using LLMs to Facilitate Group Conversations

Recent advancements in large language models (LLMs) have provided a new avenue for chatbot development. Most existing research, however, has primarily centered on single-user chatbots that determine "What" to answer. This paper highlights the complexity of multi-user chatbots, introducing the 3W design dimensions: "What" to say, "When" to respond, and "Who" to answer. Additionally, we proposed Multi-User Chat Assistant (MUCA), an LLM-based framework tailored for group discussions. MUCA consists of three main modules: Sub-topic Generator, Dialog Analyzer, and Conversational Strategies Arbitrator. These modules jointly determine suitable response contents, timings, and appropriate addressees. This paper further proposes an LLM-based Multi-User Simulator (MUS) to ease MUCA's optimization, enabling faster simulation of conversations between the chatbot and simulated users, and speeding up MUCA's early development. In goal-oriented conversations with a small to medium number of participants, MUCA demonstrates effectiveness in tasks like chiming in at appropriate timings, generating relevant content, and improving user engagement, as shown by case studies and user studies.

==> sections/future_work.tex <==
\section{Future Work}
\label{sec:future_work}

The framework we propose for multi-user chatbots is not intended as a comprehensive solution for multi-user conversations. Rather, we hope this work can shed light on potential directions for future research in the field of multi-user chatbots. Several areas, including but not limited to the following, deserve further research:

\textbf{Component Orchestration:} The proposed MUCA framework integrates several components, enabling actions such as "participation encouragement" and "initiative summarization". These components have been carefully designed, tuned, and ranked to provide a harmonious experience to the chat participants. It can be beneficial to explore an easy plug-and-play method for users to design and incorporate new components into the framework without intensive tuning. Such a feature could be important, as different conversation scenarios may require different chatbot personas.

\textbf{Human-in-the-loop Feedback Iteration:} Full user studies for feedback are costly and time-consuming. To continuously improve chatbot post-launch, it is useful to collect implicit and explicit user behavior signals. This data should be easily transformable for automatic or semi-automatic chatbot enhancements.

\textbf{Rapidly Advancing AI Technologies:} The proposed MUCA framework is based on the recent state-of-the-art LLMs, each with its unique style and best practices for prompting. It would be beneficial to investigate methods for updating the underlying AI models without the need for complete re-prompting or component orchestration.

\textbf{Multi-modal Capabilities and External Resources:} As LLMs become increasingly capable of processing multi-modal data, a chatbot that interacts with multiple users using not only text, but also video, audio, and images is becoming feasible. Additionally, external resources could be integrated as a component for the chatbot to leverage to enhance the multi-user conversation experience.

\textbf{Multi-Chatbot Design:} The study concentrates on multi-user and single-chatbot interactions, but examining scenarios with multiple users and chatbots, each having diverse personas, interacting could be intriguing.
% This study focuses on scenarios involving multiple users and a single chatbot interacting with each other. However, it could be interesting to explore applications where multiple users and multiple chatbots with different personas interacting with each other. 
For instance, in cross-disciplinary meetings, chatbots could serve as hosts, minute-takers, or subject matter experts, offering insights to human participants as needed.
